Layered Image Vectorization via Semantic Simplification

This work presents a progressive image vectorization technique that reconstructs the raster image as layer-wise vectors from semantic-aligned macro structures to finer details. Our approach introduces a new image simplification method leveraging the feature-average effect in the Score Distillation Sampling mechanism, achieving effective visual abstraction from the detailed to coarse. Guided by the sequence of progressive simplified images, we propose a two-stage vectorization process of structural buildup and visual refinement, constructing the vectors in an organized and manageable manner. The resulting vectors are layered and well-aligned with the target image's explicit and implicit semantic structures. Our method demonstrates high performance across a wide range of images. Comparative analysis with existing vectorization methods highlights our technique's superiority in creating vectors with high visual fidelity, and more importantly, achieving higher semantic alignment and more compact layered representation. The project homepage is https://szuviz.github.io/layered_vectorization/.

==> sec-old/03-overview-old.tex <==

\begin{figure}[!htb]
  \centering
    \includegraphics[width=1.\linewidth]{figures/framework6.png}
    % {img/match.png}
    \caption{Layered vectorization pipeline: to optimize the current level, primitives are initialized at regions where semantic and visual differences are most pronounced. The vector primitives are rendered and optimized by backpropagating a joint loss function, enhancing both structural representation and visual appearance. \dc{NICE FIGURE!}}
  \label{fig:framework}
\end{figure}

\section{Overview}
\label{sec:overview}

%\lmc{Danny, I updated Section 3 to the new pipeline. You can have a pass.}

Our framework consists of two modules that work sequentially to achieve layered vectorization.  One module is \textit{Progressive Image Simplification} that employs Score Distillation Sampling~\cite{poole2022dreamfusion} combined with semantic segmentation to generate a sequence of images with varying levels of semantic simplicity (see the first row in Figure~\ref{fig:vec}). The other module \textit{Layered Vectorization} uses that series of simplified images as guidance and generates vectors layer by layer, from coarse to fine level of detail (see the second to fourth rows in Figure~\ref{fig:vec}).




Figure~\ref{fig:framework} illustrates the vector optimization per simplified level. Taking the simplified image at the current level as input, we compute its differences from images from the previous levels to estimate where additional primitives should be best added. This process involves examining differences at two levels: the semantic segmentation level and the pixel level. At the semantic segmentation level, vector primitives are initialized where the segmentation differences are detected, referred to as \textit{structure-wise vector primitives}. At the pixel level, primitives can be optionally initialized (noted as \textit{pixel-wise primitives}). This primitive initialization encourages the vector representation to effectively capture both semantic and pictorial information (Section~\ref{subsec:primitive_init}).

The newly added primitives, together with the primitives from all previous levels, undergo a joint optimization towards two main losses. One is the \textit{Visual Loss}, which considers the visual fitness of the target image at the current level. The other is the \textit{Structural Loss}, which weighs the impact of shape alignment between structure-wise primitives and their corresponding semantic segmentation to ensure that the vector representation accurately maintains the essential structural semantics. As shown on the right part of Figure~\ref{fig:framework}, both losses are designed as image-space losses by leveraging the capabilities of differential rendering~\cite{li2020differentiable}. Specifically, for structural loss, we first organize structure-wise primitives into distinct layers. Then, for each layer, an MSE-based loss is computed between the rendered image of structure-wise primitives and their corresponding segmentation image. The optimization of the vector primitives is achieved by combining the structural loss from all layers together with the visual loss. Further details regarding the loss shall be provided in Section~\ref{subsec:loss_func}. Following this process, we progressively add vector primitives from one simplified level to the next. 
%\lm{Upon completion of all levels, we perform a vector organization. This process forms groups, where vectors are in a containing and contained relationship, facilitating easier manipulation and editing.}
Once all levels are computed, we organize them into groups with containing and contained relationships to facilitate easier manipulation and editing.

%We use a weight scheduler that dynamically controls when and how the structure losses join in the compound loss. There are two phases: first, primitives from previous levels are frozen and only the current level is considered to optimize the newly added primitives toward the basic appearance of desired pictorial details. Then in the second phase, all primitives are involved and optimized to approach the overall image's visual appearance at the current level. A larger weight is assigned to the loss at the current level, while smaller weights are assigned to the losses from previous levels. Incorporation of MSE losses from the previous levels is a crucial constraint in our framework, ensuring that the previously added primitives can persist to the pictorial details they are intended to represent so that they would not be glitched and shifted to other new visuals during the optimization. 

%This weighting scheme emphasizes the importance of the current level in the optimization process, allowing for a more focused and effective refinement of the vector primitives. 

%\dcc{But you could freeze the previous ones.. at least the reader would expect that}




==> sec-old/04-method-old.tex <==
\section{Semantic Simplification}
\label{sec:sds}

%\dcc{It is clear, but why you don't freeze all previous paths when you optimize the new ones. At least for a while, and then, maybe you can do the compound loss... I think it will be faster. At least try and show an ablation. Yet, I will go through the text a bit} \lmc{I get it, yes, freeze others but just optimizing the new paths can be faster. We will try it! }

%Our framework involves a process of iteratively abstracting images, followed by a process of generating vectors layer by layer, starting from the most abstract image and progressing toward the least abstract image. 

%\lmc{We include possible image abstraction techniques including Superpixel, Gaussian low-pass filter, and SDS. And we discuss their cons and pros, show SDS is better.}

%\dcc{I think it is to risky to claim and call it "abstraction". Abstraction is a very ambitious. Unless we have really convincing results, I would call it "simplification" and if we get good results we can even claim that it is "semantic simplification".} 
%\lmc{ok! yes, 'abstract' is too abstract to know what it is. I feel more easy with 'simplification' : D. I will change the text accordingly. How about 'progressive simplification'? we can add 'semantic' if SDS really are.}

%One \lm{notable} distinction that sets our work apart from existing image vectorization approaches is the concept of layered semantic simplification of images. \dcc{Are you sure, it is very strong statement} 

Our layered vectorization technique is progressively directed by a sequence of images semantically simplified from the original image. Current vectorization techniques primarily perform pixel-level analysis of the input image to decide where to add and optimize paths, such as large connected areas identified by color quantification in LIVE~\cite{ma2022towards} or clusters via DBSCAN in Optimize \& Reduce (O\&R) method~\cite{hirschorn2024optimize}. Rather than solely analyzing the original image, our approach involves generating a series of simplified images and their semantic segmented masks derived from the original. Figure~\ref{fig:sequence_example} shows an example of the simplified image sequence generated using our SDS-based method (Section~\ref{subsec:sds}). As can be seen, the image sequence exhibits varying levels of simplicity, from the original one with many intricate details and textures to a simplified and overall outline on the right.

%\dcc{Do we use "abstraction" still?} \lmc{I changed most of them to 'simplicity'.}

The intuition behind using simplified images to guide layered vectorization is to prioritize the capture of the overall structure before addressing subtle changes. This approach offers two notable benefits. Firstly, by decomposing the vectorization process into manageable levels, it becomes more tangible and achievable compared to optimizing it as a whole. The incremental improvement from one abstract level to the next is relatively small, allowing for effective optimization at each step. Secondly, the progressive abstraction establishes a coarse-to-fine hierarchy, enabling holistic optimization of delicate paths within the image. This approach becomes particularly advantageous when dealing with shapes that exhibit pixel variations due to occlusion, shadows, or textures yet remain integral components of a larger entity. For example, in the right of Figure~\ref{fig:sequence_example}, the `cat' is abstracted as a shape unit at the most simplified level, while pixel-based methods such as LIVE or O\&R would represent the cat with fragmented shapes and fail to capture the entire cat shape due to the occlusion of the `stripped sweater'. Our method favors that these paths are retrieved as complete entities, enhancing the overall editability and preserving the intended structure of the figure. 

\begin{figure}[!htb]
  \centering    \includegraphics[width=1.\linewidth]{figures/abstract_seq5.png}
    \caption{Layered simplified images: (left) a sequence of simplified images generated with our SDS method, with the original image on the leftmost as input. (right) instead of being represented by individual parts (highlighted in green), the cat shape can be captured by a single continuous path with our semantic simplification on the right. }
  \label{fig:sequence_example}
\end{figure}

\subsection{Pixel-based Simplification}

Pixel-based simplification techniques, such as Superpixel~\cite{achanta2012slic} and Gaussian low-pass filter, can serve as baseline choices for this purpose. By varying Gaussian kernels with radius from small to large, a sequence of images can be generated by reducing image noise and detail. By changing the number of superpixels, images can be simplified by various numbers of pixel groups that share common characteristics. Pixel-level simplification methods operate by manipulating the intensity values of individual pixels and their surrounding pixels. While these techniques can effectively reduce the complexity of an image, they do not consider the semantics of the objects present in the image. Consequently, as exemplified in Figure~\ref{fig:abstract_short}, when these methods are applied to high-level abstract, they may inadvertently blur or blend adjacent objects, which introduces significant problems in the contour of semantic segmentation, such as the leakage and inaccurate boundaries of the `head of the bird'.


\begin{figure}[!htb]
  \centering    
  \includegraphics[width=1.\linewidth]{figures/three_abstract_short.png}
    \caption{Compared to pixel-based simplification techniques, e.g., Gaussian blur and SuperPixels, our SDS simplification can maintain the semantics of objects well. With SDS, the boundaries of semantic segmentation are effectively smoothed while still retaining important geometric features, such as the distinct shape of the `bird's mouth'. Note that the top row displays simplified images, while the bottom row shows the corresponding semantic segmentation.}
    %A complete visualization of this example is provided in the supplement materials.}
  \label{fig:abstract_short}
\end{figure}

\subsection{Simplification with SDS}
\label{subsec:sds}

\lmc{we need to decide whether SDS is special and explain why.}

In our work, we introduce a novel semantic simplification technique that makes use of the \textit{Feature-averaged Effect} in Score Distillation Sampling (SDS)~\cite{poole2022dreamfusion}. As shown in the right column of
Figure~\ref{fig:abstract_short}, our SDS-based simplification approach effectively reduces intricate details, such as the feather texture of the bird and the background, while preserving fundamental features, such as a rough silhouette depiction of the bird. 
%although blurred, effectively simplifies the semantics of the image. For example, the simplified cake has a single fruit placed on top.


As investigated by Liang et al.~\cite{liang2023luciddreamer}, the feature-average effect of SDS can be explained by rewriting the gradient of SDS loss as:

\begin{equation}
% \nabla_\theta \mathcal{L}_{\mathrm{SDS}}(\phi, \mathbf{x}=g(\theta)) \triangleq \mathbb{E}_{t, \epsilon}\left[w(t)\left(\hat{\epsilon}_\phi\left(\mathbf{z}_t ; y, t\right)-\epsilon\right) \frac{\partial \mathbf{x}}{\partial \theta}\right],
    \nabla_\theta \mathcal{L}_{\mathrm{SDS}}(\theta)=\mathbb{E}_{t, \boldsymbol{\epsilon}}\left[\frac{\omega(t)}{\gamma(t)}\left(\boldsymbol{x}_0-\hat{\boldsymbol{x}}_0^t\right) \frac{\partial \boldsymbol{g}(\theta)}{\partial \theta}\right] ,
\end{equation}
where $g$ is the differentiable generator that transforms parameters $\theta$ to create an image $x = g(\theta)$, e.g., $g$ is a NeRF volume renderer in the original SDS work~\cite{poole2022dreamfusion}. In our work, we take $g$ as a generator that renders a single image~\cite{hertz2023delta}. Therefore, $\theta$ are the image pixels. SDS drives the input image $\boldsymbol{x}_0$ towards the $\hat{\boldsymbol{x}}_0^t$, which is averaged from the images with inconsistent features predicted by the diffusion model DDPM~\cite{ho2020denoising}. The diffusion model first perturbs $\boldsymbol{x}_0$ to $\boldsymbol{x}_t$ with random noises. However, DDPM is overly sensitive to its input, where minor fluctuations in $\boldsymbol{x}_t$ would change the details of the predicted images. A smoothed image without individual details is achieved by averaging images with local feature-inconsistent.  

% \dc{I didn't understand...I think it is ok to leave it a bit unclear, without Fig 5...}
% \lmc{Ok. updated.}

% \begin{figure}[!htb]
%   \centering    
%   \includegraphics[width=1.\linewidth]{figures/sds_average.png}
%     \caption{The inconsistent features of predicted images by DDFM are used for semantic simplification, i.e., smooth individual details while maintaining overall consistency. \lmc{I borrow this from ~\cite{liang2023luciddreamer}, we MUST change this image to ours.}}
%   \label{fig:sds_average}
% \end{figure}

We have adjusted the Guidance Scale parameter in Classifier-free Guidance (CFG)~\cite{ho2022classifier} to introduce greater variation in the generated images. Specifically, we have reduced the value of the Guidance Scale from its usual value of 7.5 to 1.0. This modification enables the diffusion model to exhibit more creativity and deviate less strictly from the given text prompt. 

By different numbers of SDS iterations, a sequence of $N$ images at different simplified levels can be generated. In our work, $N$ is set to five, i.e., the origin image and four simplified images sampled every 20 steps throughout 80 SDS iterations. As shown in Figure~\ref{fig:abstract_short}, the SDS method simplifies the image at a very abstract level while effectively maintaining the overall shape of the `bird' and `flowers'. It is important to note that although the resulting images appear blurred, they still allow for effective semantic segmentation. Moreover, the boundaries of detected objects are smoothed and compatible with vector-based graphics.

% \dc{In the above you refer to "masks", but only below you define it...}
% \lmc{remove the mask here.}

% It is important to note that while the resulting images may exhibit blurriness, their primary function is to identify areas with significant variance. These regions, characterized by unclear boundaries, will be refined and calibrated in subsequent steps of the progressive optimization using later images that possess clear boundaries.}

% \dcc{We need to admit that it is indeed blurry, but it is just used to find the location of large varience!!!}
% \lmc{I added this and how about it now?}

%\dcc{This is our biggest challenge - to prove that SDS is not an overkill here!!!!}


==> sec-old/04-vector-old.tex <==
\section{Layered Vectorization}

With the sequence of simplified images, layers of vectors are progressively added and optimized from the simplest to the most detailed. Below, we introduce the key components of this part.  

\subsection{Primitive Initialization}
\label{subsec:primitive_init}

During the optimization process of the $N^{th}$ level ($N$ valued from small to large, corresponding to the simple to the detailed), vector primitives are strategically initialized at locations where prominent differences are detected from the current image to the previous ones. We primarily consider the differences in semantics, i.e., based on the segmentation difference, and take the pixel-level difference as an additional complementary to the detailed visual effects. 

To add structure-wise primitives, semantic segmentation is first applied in the $N^{th}$ simplified image to categorize pixels into meaning regions, which we refer to as \textit{masks}. Subsequently, the masks from the $N^{th}$ are compared to the existing masks of the $N-1$ levels (as shown in the left of Figure~\ref{fig:path_init} (a)). Only the new masks that were not present in the preceding $N-1$ levels are added. If a mask from the current level exhibits a high degree of overlap with existing masks, determined using the Jaccard similarity coefficient~\cite{jaccard1901etude}, we refrain from adding it, as it likely represents the same semantic object. Once the masks are identified and added, we initialize vector primitives for each one. We use the Douglas-Peucker simplified representation of the masks as the initial shape~\cite{douglas1973algorithms}. To delicately capture the complex shapes at this stage, a closed shape composed of eight cubic Bézier curves is used as the basic vector primitive.

\begin{figure}[!htb]
  \centering    
  \includegraphics[width=1.\linewidth]{figures/path_init2.png}
    \caption{Path initialization: (a) structure-wise primitives are initialized where differences are identified between semantic segmentation of the current image and previous ones, (b) pixel-wise primitives are initialized around significant pixel-level differences between the current image to its previous one.}
  \label{fig:path_init}
\end{figure}

To add pixel-wise primitives, we compute the pixel-level difference between the $N^{th}$ simplicity level and the previous level $(N - 1)^{th}$. A connected component labeling algorithm is applied over pixels in the $N^{th}$ simplified image to connect pixels into regions with a maximum difference threshold $C_{diff}$. As shown in Figure~\ref{fig:path_init}(b), the pixel-level difference is quite intricate,  exhibiting unpredictable or irregular patterns. This suggests that it is challenging to construct a compact vector structure using purely pixel-level analysis, such as the method used in LIVE~\cite{ma2022towards}. In our work, we control the complexity of vector representation by a parameter $P_{num}$, the number of pixel-level primitives to be added per level. Also, to restrain the complexity, we employ a closed shape of four cubic Bézier curves as the fundamental pixel-wise primitive, which is more straightforward than the structure-wise primitive. 


\subsection{Loss Function}
\label{subsec:loss_func}

The loss function comprises two main components: the \textit{structural loss}, which measures the alignment of structure-wise primitives to the segmentation across layers, and the \textit{visual loss}, which assesses the visual fitness of all primitives to the simplified image at the current level.

\paragraph{\textbf{Structural Loss}}

The structural loss $\mathcal{L}_{structure}$ is computed as the sum of MSE loss over the layers $M$. For each layer $j$, the structural loss is calculated as the MSE between the rendering of structure-wise primitives at that layer $I_{layer_j}$ and their corresponding segmentation image $I_{segment_j}$. This function concentrates on optimizing shape rather than colors or any other non-spatial visual appearance. Therefore, we assign the same random color to each pair of structure-wise primitives and their corresponding segmentations. With the $MSE_j$ per layer, the structural loss is defined as: 

\begin{equation}
\mathcal{L}_{structure} = \sum_{j=1}^{M} MSE(I_{layer_j},\  I_{segment_j}). 
\end{equation}


%  \begin{figure}[!htb]
%   \centering
%     \includegraphics[width=1.\linewidth]{figures/icecream.png}
%     % {img/match.png}
%     \caption{Vectorization of an `Icecream' Image: (a) our method generates more structured vector representation, e.g., the hierarchy of `ball' and 'bowl', compared to (b) O\&R~\cite{ma2022towards} and (c) LIVE~\cite{ma2022towards}.  }
%   \label{fig:icecreem}
% \end{figure}

\paragraph{\textbf{Visual Fidelity Loss}}

A visual fidelity loss $\mathcal{L}_{fidelity}$ is used to measure the faithfulness to the input image, i.e., the rasterized vectors $I_{vector}$ has to be similar to the input target $I_{target}$. We define $\mathcal{L}_{fidelity}$ as their RBG error under $L_2$ norm: 

\begin{equation}
% \mathcal{L}_{visual} = \frac{1}{n} \sum_{i=1}^{n} (I_{render,i} - I_{target,i})^2, 
\mathcal{L}_{fidelity} = \sum_{p \in I} \| I_{target}(p) - I_{vector}(p) \|_2^2.
%MSE(I_{render}, I_{target}). 
\end{equation}

% where $I_{render}$ and $I_{target,i}$ represent the pixel intensity values at the $i^{th}$ pixel in the two images respectively. $n$ is the total number of pixels in the images.

\paragraph{\textbf{Vector Simplicity Loss}}

Another loss $\mathcal{L}_{simplicity}$ is used to maintain the simplicity of the vectors by favoring those with small perimeters, ensuring they capture the essence of the data without unnecessary detail:

\begin{equation}
\mathcal{L}_{simplicity} = \sum_{i=1}^{n} \| P_{i} - P_{i+1} \|,
%ReLU(L - L_\text{min}),
\end{equation} 

where $P$ is the control point of cubic Bézier curves, with $P_{n+1}=P_{1}$ to close the loop. 

With the above, the loss function is a joint one, as follows:

\begin{equation}    
\mathcal{L}_{\text{total}} =  \mathcal{L_{}}_{\text{fidelity}} + \beta \mathcal{L}_{\text{structure}} + \delta \mathcal{L}_\text{simplicity}.
\end{equation}

%where the parameters $\beta$ and $\delta$ are used to balance the contribution of each loss component to the total loss. This joint loss function allows the model to optimize for visual accuracy, structural integrity, and curve length simultaneously. 

%For examples shown in the paper, $\alpha$ and $\beta$ is set to 1, and $\delta$ is set to 0.1. 

% \dc{Sorry, I didn't have patient to really read Section 5...I did only some cosmetic changes. I will touch the caption of Fig 6}
% \lmc{ok ; )}







==> sec/06-implementation.tex <==
\section{Implementation}

\lmc{to be updated, to be moved to SU}

We implemented this method using PyTorch with the Adam optimizer. The learning rates for optimizing primitive points and their colors are set to 1.0 and 0.01, respectively. By default, a sequence of five simplified images is generated at intervals of 20 SDS iterations. In layered vectorization, we perform optimization through 100 iterations at each level of simplicity, except the final level. For the ultimate stage of fitting the target image, we conduct 500 iterations to achieve optimal results. At the end of each iteration, paths shorter than 25 units are removed. The initial shape of paths at the beginning of each iteration is circular with a radius of 5 units, following the approach used in LIVE. By default, we add up to 200 visual paths, with the option to customize the number of visual elements added. The $\alpha$ and $\beta$ are set to 1, and $\delta$ is set to 0.1. All examples and experiments in this paper were conducted on a system running Ubuntu 20.04.6 LTS, equipped with an Intel Xeon Gold 5320 CPU operating at 2.20 GHz and four NVIDIA A40 GPUs. Each GPU features 48 GB of GDDR6 memory with ECC.



==> sec/abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/table.tex <==
\begin{table}[h]   % 表格中不带引用
\setlength{\abovecaptionskip}{0.1cm} 
\setlength{\belowcaptionskip}{0.1cm}
\tabcolsep=1cm
\footnotesize
\renewcommand\arraystretch{1.2}  % 行间距
\setlength\tabcolsep{1.2pt}   % 列间距
\centering
\caption{Comparison among classic dataset.}
\begin{tabular}{lrccccccccc}
    \toprule[1pt]
    \multirow{2}{*}{Dataset}&\multirow{2}{*}{\# Images} & \multirow{2}{*}{\# Attributes} &\# Annotators & Model &Image\\
    &&&(per image)&(\# classes)& type\\
    \midrule[0.5pt]
    IAPSa&     390     & - & -  &Mikels (8)  & Natural          \\
    Abstract & 280     & - & 14  & Mikels (8)      & Abstract         \\
    ArtPhoto  & 806    & - & -   & Mikels (8)     & Artistic         \\
    TwitterI  & 1,269  & - & 5   & Sentiment (2)  & Social           \\
    TwitterII   & 603    & - & 3  & Sentiment (2)   & Social           \\
    Emotion6  & 1,269    & - & \textbf{15}  & Ekman (6) & Social           \\
    Flickr   & 60,745   & - & 3   & Sentiment (2)  & Social           \\
    Instagram & 42,856 & - & 3   & Sentiment (2)  & Social           \\
    FI        & 23,164    & - & 5   & Mikels (8)     & Social           \\
    EMOTIC   & 18,316   & - & 3   & Ekman (6)      & Social           \\
    \textbf{EmoSet (Ours})      & \textbf{118,102}   & \textbf{6} & 10   & Mikels (8)     &Social, Artistic\\
    \bottomrule[1pt]
\end{tabular}
\end{table}

% IAPSa
@article{mikels2005emotional,
title={Emotional category data on images from the International Affective Picture System},
author={Mikels, Joseph A and Fredrickson, Barbara L and Larkin, Gregory R and Lindberg, Casey M and Maglio, Sam J and Reuter-Lorenz, Patricia A},
journal={Behavior research methods},
volume={37},
number={4},
pages={626--630},
year={2005},
publisher={Springer}
}
%Abstract ArtPhoto
@inproceedings{machajdik2010affective,
title={Affective image classification using features inspired by psychology and art theory},
author={Machajdik, Jana and Hanbury, Allan},
booktitle={Proceedings of the 18th ACM international conference on Multimedia},
pages={83--92},
year={2010}
}
% Twitter1 
@inproceedings{you2015robust,
title={Robust image sentiment analysis using progressively trained and domain transferred deep networks},
author={You, Quanzeng and Luo, Jiebo and Jin, Hailin and Yang, Jianchao},
booktitle={Twenty-ninth AAAI conference on artificial intelligence},
year={2015}
}
% Twitter2
@inproceedings{borth2013large,
title={Large-scale visual sentiment ontology and detectors using adjective noun pairs},
author={Borth, Damian and Ji, Rongrong and Chen, Tao and Breuel, Thomas and Chang, Shih-Fu},
booktitle={Proceedings of the 21st ACM international conference on Multimedia},
pages={223--232},
year={2013}
}


% emoton6
@inproceedings{peng2015mixed,
title={A mixed bag of emotions: Model, predict, and transfer emotion distributions},
author={Peng, Kuan-Chuan and Chen, Tsuhan and Sadovnik, Amir and Gallagher, Andrew C},
booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
pages={860--868},
year={2015}
}
% Flickr2 Instagram
@inproceedings{katsurai2016image,
title={Image sentiment analysis using latent correlations among visual, textual, and sentiment views},
author={Katsurai, Marie and Satoh, Shin'ichi},
booktitle={2016 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
pages={2837--2841},
year={2016},
organization={IEEE}
}
% FI
@inproceedings{you2016building,
title={Building a large scale dataset for image emotion recognition: The fine print and the benchmark},
author={You, Quanzeng and Luo, Jiebo and Jin, Hailin and Yang, Jianchao},
booktitle={Proceedings of the AAAI conference on artificial intelligence},
volume={30},
number={1},
year={2016}
}
% EMOTIC
@inproceedings{kosti2017emotion,
title={Emotion recognition in context},
author={Kosti, Ronak and Alvarez, Jose M and Recasens, Adria and Lapedriza, Agata},
booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
pages={1667--1675},
year={2017}
}


